Science DMZ Networks: How Different are They Really?

The Science Demilitarized Zone (Science DMZ) is a network environment optimized for scientific applications. A Science DMZ provides an environment mostly free from competing traffic flows and complex security middleware such as firewalls or intrusion detection systems that often impede data transfer performance. The Science DMZ model provides a reference set of network design patterns, tuned hosts and protocol stacks dedicated to large data transfers and streamlined security postures that significantly improve data transfer performance, accelerating scientific collaborations and discovery. Over the past decade, many universities and organizations have adopted this model for their research computing. Despite becoming increasingly popular, there is a lack of quantitative studies comparing such a specialized network to conventional production networks regarding network characteristics and data transfer performance. We strive to answer the following research questions in this study: Does a Science DMZ exhibit significantly different behavior than a general-purpose campus network? Does it improve application performance compared to such general-purpose networks? Through a two-year-long quantitative network measurement study, we find that a Science DMZ exhibits lower latency, higher throughput, and lower jitter behaviors. However, we also see several non-intuitive results. For example, a DMZ may take a longer route to external destinations and experience higher latency than the campus network. While the DMZ model benefits researchers, the benefits are not automatic - careful network tuning based on specific use cases is required to realize the full potential of such infrastructure.

==> 3.0-emily.tex <==

\subsection{Path }
%ping latency
    %RIPE
When there is inbound WAN traffic from RIPE Atlas, both the campus network and the DMZ exhibit similar latency, with the campus network occasionally having a lower average latency than the DMZ by as much as $\sim$20ms (5\% - 30.5\%) (unexpected result). This result is due to a period of time in which 2 of 4 sources of the ping measurements were not arriving at the DMZ despite arriving at the campus network. 1 of the 2 sources that completed its route to the DMZ was one of typical high latency, which affected the average latency poorly as the other 3 sources typically produce much lower latency. ***Takeaway: the campus network and the DMZ usually have similar latency with inbound traffic from RIPE.
    %GCP
When traffic is inbound from Google Cloud, both nodes on the DMZ tend to have similar latency, with an occasional $\sim$2\% difference. The campus network tends to have higher latency but occasionally has similar latency to the DMZ. The campus network has a $\sim$2\% - 24\% higher latency than the DMZ.
    %External
When traffic is outbound to perfSONAR nodes, both nodes on the DMZ exhibit similar latency while the campus network experiences latency that is 30.43\% - 83\% slower.

%packet loss
    %RIPE
When there is inbound traffic from RIPE Atlas, the DMZ experiences more spikes of packet loss than the campus network. While the campus network exhibits a period of 100\% packet loss due to the campus node being down, both nodes of the DMZ experience 50\% genuine packet loss. The Perfsonar1 node on the DMZ exhibits more instances of packet loss than the DTN1 node on the DMZ; it loses $\sim$5\% more packets than DTN1 over 3 months. ***Should quantify campus-dmz loss comparison, but not sure how to approach it yet***
    %GCP
When traffic is incoming from Google Cloud, there is no pattern of packet loss across DMZ or campus network.
    %External
When traffic is outbound to external perfSONAR nodes, the campus network experiences more packet loss than the DMZ as a whole, but the Perfsonar1 node experiences more packet loss than the DTN1 node. Perfsonar1 exhibits $\sim$2\% more packet loss than DTN1. The campus network exhibits $\sim$4.2\% more packet loss than Perfsonar1 and $\sim$5.7\% more packet loss than DTN1.

%jitter
    %RIPE
    When traffic is inbound from RIPE Atlas, Leo exhibits lower average jitter than the DMZ nodes. Jitter on the Leo route tends to be 60-78\% lower than on the DMZ routes, but also exhibits the same level of jitter as the DMZ nodes at multiple points. DTN1 tends to exhibit higher variation in its daily jitter than Perfsonar1, by as much as 37 milliseconds.
    %GCP
    When traffic is inbound from GCP to Leo and the DMZ nodes, all three routes exhibit similar average jitter patterns between 0-1 milliseconds, only ever differing by fractions of milliseconds. Leo's route often experiences more deviation in its jitter than the DMZ nodes by as much as 2 milliseconds. The DTN1 node experiences more deviation than the Perfsonar1 node by as much as 1.5 milliseconds.
    %External
    When traffic is outbound to perfSONAR nodes, Leo and the DMZ nodes usually have an average jitter between 0-1 milliseconds. But Leo often reaches higher jitter rates up to 10-63 milliseconds greater than the DMZ nodes.
%traceroute hops and latency
    %RIPE (excluded hops of 2 because it is not architecturally possible)
    When traffic is inbound from RIPE Atlas, the range of hops is the same to get to Leo and the two DMZ nodes. Comparing only common hop counts, both nodes on the DMZ have similar latency except for when the route averages 16 hops. At that point, the DTN1 node has 11\% lower latency.  Both DMZ nodes often exhibit 34-73\% lower latency than Leo, but Leo has path lengths that are 13-30\% lower latency than the DMZ nodes. 
    
    %GCP
When traffic is inbound from Google Cloud, the campus network experiences a route path that is one hop shorter than the routes that the DMZ nodes take. But the DMZ exhibits lower latency at all route lengths in common with the campus network by $\sim$3\% - 6.78\%.
    %External
When traffic is outbound to external perfSONAR nodes, the campus network experiences routes with ranges 1-2 hops shorter than DMZ routes. But, the DMZ tends to have a latency 20\% - 36.7\% lower than the campus network (gathered from common path lengths observed through traceroute). However, there is a point when the campus network performs faster than the DMZ by 12.5\% at 10 hops. The DTN1 node on the DMZ has a latency, at the longest path length, that is $\sim$6.75\% lower than that of the Perfsonar1 node on the DMZ.

%throughput
When measuring throughput between Google Cloud and the campus nodes, Leo typically exhibits 2-89\% lower upload throughput than Perfsonar1 and download throughput 0.3-88\% lower. However, there is a period at the beginning of the measurement study where Perfsonar1 exhibits upload throughput 2-4\% lower than Leo and download throughput 1-4\% lower.

\subsection{LAN Results}
%ping latency
During traffic between local nodes, the DMZ routes have significantly lower latency than the campus network. The DMZ’s reported RTT is 80\% - 99.5\% (0.8 - 2998 ms) lower than that of the campus network’s route. The route from DTN1 to DTN2 has 33\% - 61.2\% lower latency than the route from DTN1 to Perfsonar1.
%gateway latency
Traffic from the Perfsonar1 node on the DMZ to the campus gateway node has a 8-50\% (0.1 - 20 ms) lower latency than traffic from the Leo node on the campus network to the campus gateway node.
%packet loss
During local traffic between local network nodes, the campus network node loses more packets than the DMZ nodes. The campus network loses $\sim$2.3\% more packets than the DMZ over the course of three months.
%jitter
Jitter between DMZ nodes tend to have an average jitter between 0 and 0.1 milliseconds. But the route from Leo to the Perfsonar1 node on the DMZ reaches jitter rates up to 66 milliseconds. The Leo route tends to have deviation 10-3500 times greater than deviation exhibited by the DMZ nodes. The route from DTN1 to Perfsonar1 exhibits higher deviation in jitter than the route from DTN1 to DTN2 by as much as 2.5 times higher.
%traceroute hops and latency (may leave this out because it does not offer much insight)

\subsection{BGP Results}

\subsection{Data Transfer Results}
%Interarrival Interpacket Delay
The average delay between packets tends to be 63-80\% lower when downloading on DTN1 than on Leo.

%RTT
The average round-trip time from the file source to DTN1 tends to be 35-83\% lower than from the file source to Leo.

%Throughput
The average throughput observed from Leo is 93-95\% lower than that observed from DTN1. The DTN1 node successfully transmits/accepts 15-21 times more traffic than Leo.

%Total Download Time
DTN1 downloads files in 94-98\% less time than Leo.

%Window Size
DTN1 tends to have a higher average outgoing window size than Leo, by 0.84-99\%. However, Leo can achieve a higher window size than DTN1 as well, by 98\% in this measurement set.
DTN1 also tends to have a higher average receiving window size than Leo, by 0.60-91\%. But, as with the outgoing window size, Leo can achieve a higher window size than DTN1 by nearly 99\%.


==> images/bgp_figures.tex <==
\begin{figure*}[!htbp]
    \centering
    % Define variables for image file names
    \def\imageA{images/BGP_HOP_COUNT.png}
    \def\imageB{images/BGP_HOP_COUNT_2.png}
    
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[width=\linewidth]{\imageA}
        \caption{BGP Path Lengths}
        \label{fig:bgp1}
\end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[width=\linewidth]{\imageB}
        \caption{BGP Path Lengths}
        \label{fig:bgp2}
\end{subfigure}


\end{figure*}


==> images/test-figure1.tex <==
\begin{figure*}[!htbp]
    \centering
    % Define variables for image file names
    % [Your image definitions remain the same]

    \subfloat[Latency and Path Lengths from RIPE Atlas to Leo]{
    \includegraphics[width=0.3\textwidth]{\imageG}
        \label{fig:wan1_hops}
    
    \hfill
    \subfloat[Latency and Path Lengths from RIPE Atlas to perfSONAR1]{
    \includegraphics[width=0.3\textwidth]{\imageH}
        \label{fig:wan3_hops}
    }
    \hfill
    \subfloat[Latency and Path Lengths from RIPE Atlas to DTN1]{
    \includegraphics[width=0.3\textwidth]{\imageI}
        \label{fig:wan5_hops}
    }
    
    \vspace{\baselineskip} % Add some vertical space between rows

    \subfloat[Latency and Path Lengths from GCP to Leo]{
        \includegraphics[width=0.3\textwidth]{\imageD}
        \label{fig:wan2_hops}
    }
    \hfill
    \subfloat[Latency and Path Lengths from GCP to perfSONAR1]{
        \includegraphics[width=0.3\textwidth]{\imageE}
        \label{fig:wan4_hops}
    }
    \hfill
    \subfloat[Latency and Path Lengths from GCP to DTN1]{
        \includegraphics[width=0.3\textwidth]{\imageF}
        \label{fig:wan6_hops}
    }

    \vspace{\baselineskip} % Add vertical space

    \subfloat[Latency and Path Lengths from Leo to external perfSONAR nodes]{
        \includegraphics[width=0.3\textwidth]{\imageA}
        \label{fig:wan7_hops}
    }
    \hfill
    \subfloat[Latency and Path Lengths from perfSONAR1 to external perfSONAR nodes]{
        \includegraphics[width=0.3\textwidth]{\imageB}
        \label{fig:wan8_hops}
    }
    \hfill
    \subfloat[Latency and Path Lengths from DTN1 to external perfSONAR nodes]{
        \includegraphics[width=0.3\textwidth]{\imageC}
        \label{fig:wan9_hops}
    }

    % Optional: Overall caption for the entire figure
    % \caption{Overall caption for all subfigures.}
    % \label{fig:all_subfigures}

\end{figure*}


==> images/throughput.tex <==
\begin{figure*}[!htbp]
    \centering
    % Define variables for image file names
    \def\imageB{images/DOWNLOAD_THROUGHPUT.png}
        \def\imageA{images/UPLOAD_THROUGHPUT.png}

    
    \begin{subfigure}[t]{0.24\textwidth}
        \includegraphics[width=\linewidth]{\imageA}
        \caption{Average daily throughput observed from iperf3 experiments to GCP}
        \label{fig:iperf_upload}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}[t]{0.24\textwidth}
    %     \includegraphics[width=\linewidth]{\imageB}
    %     \caption{Average daily download throughput observed from iperf3 experiments to GCP}
    %     \label{fig:iperf_download}
    % \end{subfigure}


\end{figure*}
